GroupChat-Bench: Benchmarking LLM Agents on Long-Term Understanding of Realistic Group Chats

Large language model (LLM) agents are increasingly expected to participate in persistent group communication, yet existing dialogue benchmarks largely focus on short, dyadic, or single-session interactions. We introduce GroupChat-Bench, a benchmark for evaluating long-term understanding in scripted multi-party dialogues that serve as a proxy for group chats. Built from TV show scripts to avoid privacy concerns, each conversation stream spans five consecutive seasons and approximately 1,300 sessions. The benchmark tests whether agents can track participant-specific information, interpersonal relationships, and contextual changes over time. Its question pools combine refined fan-quiz-style questions with template-based questions generated from temporal knowledge graphs. Agents are evaluated as dialogue sessions unfold chronologically, with access only to the conversation history available when each question is posed. To probe the influence of memorized knowledge, GroupChat-Bench includes unanswerable questions and settings with new or swapped character names. We also propose GroupChat-Mem, which combines structured memory with a raw session repository. Experiments reveal limitations in existing memory systems, while GroupChat-Mem provides a stronger baseline. Code and data are available at https://github.com/jwyang21/groupchat_bench/.

==> algorithms/simulator_alg.tex <==
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% \setlength{\textfloatsep}{5pt}
% \setlength{\belowcaptionskip}{5pt}

% \begin{algorithm}[t]
% \small
% \caption{\simname}
% \label{algo}
% \begin{algorithmic}[1]
% \REQUIRE $\mathcal{D}=\{\mathcal{S}_i\}_{i=1}^{N}$, Time interval $t$, Agent 
% \ENSURE  \(C / T\) (CorrectAnswers / TotalQuestions)

% \STATE $C$ $\leftarrow$ 0 // CorrectAnswers
% \STATE $T$ $\leftarrow$ 0 // TotalQuestions
% \STATE $\mathcal{M}_{1, 0} \leftarrow \phi$
% \FOR{$n \leftarrow 1$ \TO $N$}
%     \IF{$|Characters(\mathcal{S}_n)| < 2$}
%         \STATE \textbf{continue}
%     \ELSE
%         \STATE $u_{n, m} \leftarrow SelectQuestionTiming(\mathcal{S}_n)$
%         \STATE $c \leftarrow RandCharInThreeTurn(u_{n, m})$
%         \STATE $q_{n, m, c}, a_{true} \leftarrow RandomQnA(n, m, c)$
%         \STATE $T$ $\leftarrow$ $T$ + 1
%         \FOR{$k \leftarrow 1$ \TO $|\mathcal{S}_n|$}
%             \STATE $\mathcal{M}_{n, k} \leftarrow UpdateMemory(\mathcal{M}_{n, k-1},$
%             \STATE$u_{n, k}, d_n, t)$
%             \IF{$k = m$}
%                 \STATE $a_{n, m} \leftarrow AgentAnswer(\mathcal{M}_{n, m},$
%                 \STATE $q_{n, m, c}, d_n, t)$
%                 \IF{$a_{n, m} = a_{true}$}
%                     \STATE $C$ $\leftarrow$ $C$ + 1
%                 \ENDIF
%             \ENDIF
%             \STATE $\mathcal{M}_{n+1, 0} \leftarrow \mathcal{M}_{n, k}$
%         \ENDFOR
%     \ENDIF
% \ENDFOR


% \end{algorithmic}
% \end{algorithm}


\setlength{\floatsep}{5pt}
\setlength{\textfloatsep}{5pt}
\setlength{\intextsep}{3pt}
\setlength{\belowcaptionskip}{3pt}


% \setlength{\textfloatsep}{0pt}
% \setlength{\belowcaptionskip}{0pt}

\SetNlSty{}{\small}{:} % 굵은 글꼴과 크기 조정
\SetAlgoSkip{1.2em}
% \SetNlSkip{0.8em} % 라인 번호와 텍스트 간의 간격 조정

\begin{algorithm}[h]
\small
\caption{\simname}\label{algo}
\KwIn{$\mathcal{D}=\{\mathcal{S}_i\}_{i=1}^{N}$, Time interval $t$, System}
\KwOut{\(C / T\) (CorrectAnswers / TotalQuestions)}

$C$ $\leftarrow$ 0 // CorrectAnswers\;
$T$ $\leftarrow$ 0 // TotalQuestions\;
$\mathcal{M}_{1, 0} \leftarrow \phi$\;

\For{$n \leftarrow 1$ \textbf{to} $N$}{
    \If{$|Characters(\mathcal{S}_n)| < 2$}{
        \textbf{continue}
    }
    \Else{
        $u_{n, m} \leftarrow SelectQuestionTiming(\mathcal{S}_n)$\;
        $c \leftarrow RandCharInThreeTurns(u_{n, m})$\;
        $q_{n, m, c}, a_{true} \leftarrow RandomQnA(n, m, c)$\;
        $T$ $\leftarrow$ $T$ + 1\;
        \For{$k \leftarrow 1$ \textbf{to} $|\mathcal{S}_n|$}{
            $\mathcal{M}_{n, k} \leftarrow UpdateMemory(\mathcal{M}_{n, k-1},$
            $u_{n, k}, d_n, t)$\;
            \If{$k = m$}{
                $a_{n, m} \leftarrow SystemAns(\mathcal{M}_{n, m},$
                $q_{n, m, c}, d_n, t)$\;
                \If{$a_{n, m} = a_{true}$}{
                    $C$ $\leftarrow$ $C$ + 1\;
                }
            }
            $\mathcal{M}_{n+1, 0} \leftarrow \mathcal{M}_{n, k}$\;
        }
    }
}
\end{algorithm}



==> contents/dialsim.tex <==
Building on \dataname, \simname~features an agent taking on the role of a main character in a dialogue.
Throughout the simulation, the agent is asked questions by other characters that must be answered accurately.


% \setlength{\textfloatsep}{3pt}
% \setlength{\belowcaptionskip}{3pt}

\SetNlSty{}{\small}{:} 
\SetAlgoSkip{1.2em}

\begin{algorithm}[t]
\small
\caption{\simname}\label{alg:sim_algorithm}
\KwIn{$\mathcal{D}=\{\mathcal{S}_i\}_{i=1}^{N}$, Time interval $t$, Agent}
\KwOut{\(C / T\) (Correct / Total Questions)}

$C$ $\leftarrow$ 0 // CorrectAnswers\;
$T$ $\leftarrow$ 0 // TotalQuestions\;
$\mathcal{M}_{1, 0} \leftarrow \phi$\;

\For{$n \leftarrow 1$ \textbf{to} $N$}{
    \If{$|Characters(\mathcal{S}_n)| < 2$}{
        \textbf{continue}
    }
    \Else{
        $u_{n, m} \leftarrow SelectAskTiming(\mathcal{S}_n)$\;
        $c \leftarrow RandCharacter(u_{n, m})$\;
        $q_{n, m, c}, a_{true} \leftarrow RandQnA(n, m, c)$\;
        $T$ $\leftarrow$ $T$ + 1\;
        \For{$k \leftarrow 1$ \textbf{to} $|\mathcal{S}_n|$}{
            $\mathcal{M}_{n, k} \leftarrow UpdateMem(\mathcal{M}_{n, k-1},$
            $ u_{n, k}, d_n, t)$\;
            \If{$k = m$}{
                $a_{n, m} \leftarrow AgentAns(\mathcal{M}_{n, m},$
                $q_{n, m, c}, d_n, t)$\;
                \If{$a_{n, m} = a_{true}$}{
                    $C$ $\leftarrow$ $C$ + 1\;
                }
            }
            $\mathcal{M}_{n+1, 0} \leftarrow \mathcal{M}_{n, k}$\;
        }
    }
}
\end{algorithm}

\newcolumntype{C}{>{\centering\arraybackslash}m{3cm}}
\begin{table*}[t]
\vspace{-1mm}
% \vspace{2mm}
\renewcommand{\arraystretch}{1.15}
\centering
 \resizebox{\textwidth}{!}{
\begin{tabular}{c l c c c c c c c} 
\toprule 
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
\multirow{4}{*}{API} 
& GPT-4o-mini & 48.11 (1.26) & \textbf{35.46 (0.91)} & \underline{52.11 (0.52)} & \textbf{44.15 (2.35)} & \textbf{41.29 (0.30)} & \textbf{45.47 (2.08)} & 42.78 (1.03) \\
& GPT-4.1-nano & 26.01 (0.42) & 25.54 (1.13) & \underline{31.03 (2.36)} & 25.42 (1.48) & 29.50 (2.50) & 27.63 (0.97) & 26.44 (0.58) \\
& Gemini 2.5 Flash & \underline{\textbf{53.94 (1.26)}} & 30.86 (0.97) & \textbf{52.92 (1.66)} & 24.27 (2.01) & 37.16 (0.45) & 42.40 (1.15) & 23.75 (1.57) \\
& Gemini 2.0 Flash & 48.15 (0.68) & 29.46 (2.03) & \underline{51.02 (1.85)} & 23.67 (0.16) & 35.93 (0.42) & 42.02 (2.00) & 22.35 (0.91) \\
\midrule
\multirow{13}{*}{Open} 
& Llama 3.3-70B & 34.65 (1.58) & 27.80 (4.43) & 44.91 (2.31) & 37.63 (0.69) & 38.70 (1.75) & 39.63 (1.51) & \underline{\textbf{45.30 (1.14)}} \\
& Llama 3.1-8B & 34.31 (3.57) & 24.56 (0.87) & \underline{38.23 (1.70)} & 30.44 (1.31) & 24.61 (1.12) & 37.21 (0.95) & 32.95 (0.58) \\
& Mixtral-8x7B & \underline{38.65 (0.37)} & 26.82 (0.51) & 37.87 (2.36) & 31.10 (0.57) & 30.35 (2.14) & 32.61 (2.42) & 26.99 (0.47) \\
& Mistral-7B & 28.48 (0.58) & 27.71 (0.89) & \underline{37.85 (1.01)} & 34.31 (0.26) & 30.01 (1.20) & 34.99 (0.63) & 32.61 (1.42) \\
& Qwen 3-32B & 40.95 (3.35) & 30.82 (0.49) & \underline{47.55 (1.29)} & 36.40 (1.36) & 36.44 (1.92) & 42.87 (0.78) & 44.66 (0.42) \\
& Qwen 3-8B & 28.18 (1.25) & 30.01 (0.58) & \underline{40.19 (1.66)} & 35.55 (2.48) & 35.25 (1.01) & 36.78 (1.09) & 34.70 (0.57) \\
& Qwen 2.5-14B & 12.39 (0.28) & 21.75 (1.78) & \underline{34.40 (2.48)} & 26.69 (0.45) & 24.35 (1.93) & 30.57 (3.21) & 25.97 (2.29) \\
& Qwen 2.5-7B & 12.43 (1.33) & 24.14 (0.81) & 27.93 (1.16) & 22.22 (0.99) & 26.82 (0.73) & \underline{29.29 (1.85)} & 23.84 (1.00) \\
& Phi 4-14B & 22.86 (1.54) & 24.44 (1.44) & \underline{33.25 (1.67)} & 30.10 (0.94) & 30.95 (1.66) & 28.69 (1.19) & 29.50 (0.38) \\
& Phi 4 mini-3.8B & 10.47 (0.85) & 25.29 (2.08) & \underline{31.16 (1.78)} & 20.99 (0.99) & 30.95 (0.63) & 24.27 (2.26) & 19.75 (0.39) \\
& OLMo 2-7B & 24.61 (1.33) & 23.37 (0.68) & 13.11 (0.87) & 24.52 (4.27) & \underline{30.35 (0.37)} & 27.16 (1.12) & 28.86 (1.01) \\
& OLMoE-1B-7B & 17.97 (0.68) & 25.54 (2.18) & 6.90 (0.68) & 17.41 (6.67) & \underline{31.42 (0.28)} & 23.58 (2.35) & 27.71 (0.38) \\
& Tülu 3-8B & 24.48 (1.09) & 25.59 (0.97) & 32.10 (1.17) & 30.23 (0.47) & \underline{32.35 (0.52)} & 31.59 (0.69) & 29.63 (0.10) \\

\midrule
& Random Guessing & 20.00 & 20.00 & 20.00 & 20.00 & 20.00 & 20.00 & 20.00\\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{The performance of the agents on Friends dialogue in \simname. We conducted experiments three times and reported the accuracy and standard deviations. \textbf{Bold} indicates the best performance per retrieval method. \underline{Underline} indicates the highest score for each model.}
\vspace{-4mm}
\label{mainres}
\end{table*}

Algorithm~\ref{alg:sim_algorithm} outlines the simulation process of \simname, designed to emulate a conversation. In this simulator, each participant's utterance (including the agent's) occurs, and the agent should update its memory.\footnote{The memory can be incrementally updated in various ways (\textit{e.g.}, by storing each utterance separately or by summarizing the session up to the current utterance). A detailed discussion of these methods is provided in \S~\ref{sec4.2}.} 
During the simulation, other characters ask questions (selected from \dataname) to the agent (Line 9-11), except in sessions where the agent is the only one talking (Line 5-6).
The timing to ask a question is chosen randomly within the session (Line 9), and the speaker who asks the question is also chosen randomly. However, to make the simulation realistic, it is crucial to ensure that the chosen speaker is still present and hasn't left the session. 
We achieved this by randomly choosing from characters who were present within three turns of the agent's last utterance (Line 10). Then, a question is randomly selected and asked in the style of the corresponding speaker (Line 11). 
The agent then must respond to the question using its memory (Line 16).
The prompt for the response is created by combining the question with the dialogue history stored in the memory. 
% The prompt we used is provided in Appendix~\ref{app:promptexample}.
















==> tabs/adversarial_test.tex <==
\newcommand{\redcol}[1]{\textcolor{red}{#1}}

\newcolumntype{C}{>{\centering\arraybackslash}m{3cm}}
\begin{table}[t]
\renewcommand{\arraystretch}{1.1}
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{l c c c} 
\toprule
\textbf{Model} & \textbf{Original} & \textbf{Swapping Names} & \textbf{New Names} \\
\midrule
GPT-4o-mini & 49.21 & 38.40 (\redcol{$\downarrow$10.81}) & 46.57 (\redcol{$\downarrow$2.64}) \\
Llama3.1-70B & 48.49 & 39.00 (\redcol{$\downarrow$9.49}) & 44.27 (\redcol{$\downarrow$4.22}) \\
Llama3.1-8B & 35.59 & 31.59 (\redcol{$\downarrow$4.00}) & 32.23 (\redcol{$\downarrow$3.36}) \\
Mixtral-8x7B & 46.47 & 37.72 (\redcol{$\downarrow$8.75}) & 39.98 (\redcol{$\downarrow$6.49}) \\
Mistral-7B & 35.09 & 30.65 (\redcol{$\downarrow$4.44}) & 34.59 (\redcol{$\downarrow$0.50}) \\
\bottomrule
\end{tabular}
\end{adjustbox}

\vspace{-3mm}
\caption{The performance of the top-performing open-source agents on the adversarial test (without time limit). Numbers in parentheses represent the performance drop compared to the original test. The full experimental results are provided in Appendix~\ref{app:adversarial}.}
\label{adversarialtest}
% \vspace{-2mm}
\end{table}

==> tabs/app_original_infinite.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}m{3cm}}
\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}
\centering
\begin{adjustbox}{max width=\textwidth} 
\begin{tabular}{c l c c c c c c c} 
\toprule 
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
\multirow{3}{*}{API} & GPT-4o-mini & 38.91 (0.99)$^\dagger$ & \textbf{34.44 (0.52)} & \textbf{49.21 (0.12)} & 42.23 (1.57) & 38.91 (0.74) & \textbf{43.64 (0.42)} & 42.40 (0.99) \\
& GPT-3.5 & 31.81 (1.33) & 26.91 (2.30) & 39.45 (1.40) & 32.77 (1.31) & 32.41 (0.96) & 35.78 (0.74) & 35.98 (1.75)\\
 & Gemini 1.0 pro & 28.36 (0.97) & 28.10 (1.08) & 39.90 (1.08) & 34.11 (1.64) & 34.26 (2.91) & 30.93 (2.17) & 33.96 (2.11) \\
 \midrule
\multirow{9}{*}{Open} & \textsc{Tülu} 2-70B & 3.31 (0.32) & 29.87 (0.65) & 35.87 (2.56) & 34.72 (1.63) & 37.07 (0.72) & 33.63 (1.32) & 38.62 (1.94) \\
 & \textsc{Tülu} 2-7B & 1.57 (0.12) & 28.93 (2.81) & 28.72 (1.80) & 30.86 (2.29) & 34.55 (0.47) & 31.04 (0.96) & 32.12 (0.75) \\
 & Llama3.1-70B & 36.36 (0.68)$^\dagger$ & 31.84 (1.29) & 43.17 (0.99) & \textbf{43.81 (0.94)} & \textbf{39.85 (2.08)} & 43.17 (0.68) & \textbf{48.49 (0.97)}\\
 & Llama3.1-8B & 28.78 (0.34)$^\dagger$ & 29.89 (1.56) & 34.70 (1.75) & 33.93 (1.76) & 31.63 (2.17) & 32.91 (0.51) & 35.59 (1.09)\\
 & Mixtral-8x7B & \textbf{42.19 (1.76)} & 31.84 (0.78) & 46.47 (1.75) & 32.31 (1.09) & 35.51 (0.19) & 41.24 (2.90) & 34.18 (0.96)\\
 & Mistral-7B & 32.93 (0.59) & 28.20 (1.17) & 35.09 (1.76) & 30.16 (1.82) & 30.12 (1.45) & 31.00 (1.93) & 30.80 (1.75) \\
 & Gemma-7B & 18.78 (0.87) & 22.26 (1.52) & 23.62 (2.09) & 19.83 (1.74) & 25.07 (0.49) & 22.48 (0.25) & 20.08 (0.76) \\
 & Gemma-2B & 1.16 (0.26) & 25.03 (1.54) & 24.64 (1.31) & 24.84 (2.05) & 28.06 (1.38) & 24.56 (2.60) & 28.28 (1.94) \\
\bottomrule
\vspace{-4mm}
\end{tabular}
\end{adjustbox}
% \vspace{-3mm}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\caption{The performance of the agents on Friends dialogue in \simname (without time limit). We conducted experiments three times and reported the accuracy and standard deviations.}
\label{appfriendsinfinite}
\end{table*}

==> tabs/app_prompt_example.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|}
\hline
\multicolumn{1}{|c|}{Prompt for Response Generation} \\ \hline
\begin{tabular}[c]{@{}l@{}}You are \textless{}\textless{}\textless{}Chatbot\textgreater{}\textgreater{}\textgreater{}, a long-term conversational agent capable of interacting with multiple users.\\ Based on the {[}Retrieved Dialogue History{]} provided, please answer the given {[}Question{]}. \\ Note the following points: \\ 1. Your answer must exclusively be one of the options: (A), (B), (C), (D), (E). \\ 2. Your responses should solely rely on the retrieved dialogue history. If the information in the dialogue\\ history is insufficient to answer the question, you must choose (E). \\ 3. This question is being asked in the context of \textless{}\textless{}\textless{}Date\textgreater{}\textgreater{}\textgreater{}. \\ \\ {[}Retrieved Dialogue History{]}\\ \textless{}\textless{}\textless{}Dialog\_History\textgreater{}\textgreater{}\textgreater{} \\ {[}Question{]} \textless{}\textless{}\textless{}Question\textgreater{}\textgreater{}\textgreater{} \\ {[}Answer{]} \\ \end{tabular} \\ \hline
\end{tabular}%
}
\caption{
In the \textless{}\textless{}\textless{}Chatbot\textgreater{}\textgreater{}\textgreater{} placeholder, the name of the main character (\textit{i.e.}, Ross, Sheldon, Michael) for each TV show is inserted. In the \textless{}\textless{}\textless{}Date\textgreater{}\textgreater{}\textgreater{} placeholder, the date of the session in which the question is being asked is inserted. In the \textless{}\textless{}\textless{}Dialog\_History\textgreater{}\textgreater{}\textgreater{} placeholder, the dialogue history that the agent will use is inserted. In the \textless{}\textless{}\textless{}Question\textgreater{}\textgreater{}\textgreater{} placeholder, the question that the agent should answer along with five choices is inserted.
\label{tab:prompt_qa}
}
\end{table*}





\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|}
\hline
\multicolumn{1}{|c|}{Prompt for Response Generation} \\ \hline
\begin{tabular}[c]{@{}l@{}}You are Ross, a long-term conversational agent capable of interacting with multiple users. \\ Based on the {[}Retrieved Dialogue History{]} provided, please answer the given {[}Question{]}. \\ Note the following points: \\ 1. Your answer must exclusively be one of the options: (A), (B), (C), (D), (E). \\ 2. Your responses should solely rely on the retrieved dialogue history. If the information in the dialogue\\ history is insufficient to answer the question, you must choose (E). \\ 3. This question is being asked in the context of {[}February 26, 1999{]}. \\ \\ {[}Retrieved Dialogue History{]}\\ 
\\{[}Session \#1 on September 22, 1994{]}
\\\textless{}\textless{}Session Omitted\textgreater{}\textgreater{}
\\Ross:  No, go on! It's Paul the Wine Guy!
\\Phoebe: What does that mean?   Does he sell it, drink it, or just complain a lot? 
\\Monica: Hi, come in! Paul, this is.. ... everybody, everybody, this is Paul.
\\All: Hey! Paul! Hi! The Wine Guy! Hey!
\\Chandler: I'm sorry, I didn't catch your name. Paul, was it?
\\Monica: Okay, umm-umm, I'll just--I'll be right back, I just gotta go ah, go ah…
\\Ross: A wandering?
\\Monica: Change!  Okay, sit down.  Two seconds.
\\Phoebe: Ooh, I just pulled out four eyelashes. That can't be good.
\\\textless{}\textless{}Session Omitted\textgreater{}\textgreater{}\\

\\{[}Session \#2 on May 20, 1998{]}
\\\textless{}\textless{}Session Omitted\textgreater{}\textgreater{}
\\Rachel: Umm, hi!
\\Ross: Hi.
\\Rachel: Is Monica around? I-I have to ask her something.
\\Ross: She's doing her laundry.
\\\textless{}\textless{}Session Omitted\textgreater{}\textgreater{}
\\Rachel: Y'know what Ross? You're not going anywhere. You're gonna sit right here. \\I'm gonna make you a cup of tea and we're gonna talk this thing whole out. All right?  Hey, Dave!
\\Dave: Yeah?
\\Rachel: Umm, listen, I'm gonna need to take a rain check, my roommate is just really sick. \\Okay? Bye!  Honey, listen, I know, I know things seem so bad right now.\\

\\ {[}Question{]} Chandler: So, just for a little stroll down memory lane, Rachel was bunking with someone in May 1998. \\Any wild guesses on who was dating this mystery cohabitant by September 22, 1994? 
\\(A) Paolo (B) Paul (C) Roger (D) Vince (E) I don’t know. \\ {[}Answer{]} \\ \end{tabular} \\ \hline
\end{tabular}%
}
\caption{
An actual example of the prompt for response generation.
\label{tab:actual_prompt_qa}
}
\end{table*}

==> tabs/app_question_templates.tex <==

\begin{table*}[h]
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{llll}
\hline
\textbf{Question Type} & \textbf{Relation} &\textbf{Template} & \textbf{Question Example}\\ \hline
\multirow{32}{*}{\textbf{Without Time}} & alumni & Who is $\{\text{sub}\}$'s alumni? & Who is Lincoln High School's alumni? \\ \cline{2-4} 
 & boss & Who is $\{\text{sub}\}$'s boss? & Who is Chandler's boss? \\ \cline{2-4} 
 & \text{sub}ordinate & Who is $\{\text{sub}\}$'s \text{sub}ordinate? & Who is Chandler's \text{sub}ordinate? \\ \cline{2-4} 
 & client & Who is $\{\text{sub}\}$'s client? & Who is Chandler's client? \\ \cline{2-4} 
 & neighbor & Who is $\{\text{sub}\}$'s neighbor? & Who is Chandler's neighbor? \\ \cline{2-4} 
 & roommate & Who is $\{\text{sub}\}$'s roommate? & Who is Chandler's roommate? \\ \cline{2-4} 
 & ex-roommate & Who is $\{\text{sub}\}$'s ex-roommate? & Who is Chandler's ex-roommate? \\ \cline{2-4} 
 & fiance  & Who is $\{\text{sub}\}$'s fiance? & Who is Rachel's fiance? \\ \cline{2-4} 
 & fiancee  & Who is $\{\text{sub}\}$'s fiancee? & Who is Ross's fiancee? \\ \cline{2-4} 
 & ex-fiance  & Who is $\{\text{sub}\}$'s ex-fiance? & Who is Rachel's ex-fiance? \\ \cline{2-4} 
 & ex-fiancee  & Who is $\{\text{sub}\}$'s ex-fiancee? & Who is Ross's ex-fiancee? \\ \cline{2-4} 
 & pet  & Who is $\{\text{sub}\}$'s pet? & Who is Ross's pet? \\ \cline{2-4} 
 & dating with  & Who is dating $\{\text{sub}\}$? & Who is dating Ross? \\ \cline{2-4} 
 & job  & What is $\{\text{sub}\}$'s job? & What is Ross's job? \\ \cline{2-4} 
 & place of work  & Where does $\{\text{sub}\}$ work? & Where does Ross work? \\ \cline{2-4} 
 & age  & How old is $\{\text{sub}\}$? & How old is Ross? \\ \cline{2-4} 
 & major  & What is $\{\text{sub}\}$'s major? & What is Ross's major? \\ \cline{2-4} 
 & mother  & Who is $\{\text{sub}\}$'s mother? & Who is Ross's mother? \\ \cline{2-4}
 & father  & Who is $\{\text{sub}\}$'s father? & Who is Ross's father? \\ \cline{2-4}
 & place of birth  & Where was $\{\text{sub}\}$ born? & Where was Ben born? \\ \cline{2-4}
 & hometown  & Where is $\{\text{sub}\}$'s hometown? & Where is Monica's hometown? \\ \cline{2-4}
 & date of birth  & When was $\{\text{sub}\}$ born? & When was Ben born? \\ \cline{2-4}
 & husband  & Who is $\{\text{sub}\}$'s husband? & Who is Emily's husband?  \\ \cline{2-4}
 & wife  & Who is $\{\text{sub}\}$'s wife? & Who is Ross's wife? \\ \cline{2-4}
 & girlfriend  & Who is $\{\text{sub}\}$'s girlfriend? & Who is Joey's girlfriend? \\ \cline{2-4}
 & boyfriend  & Who is $\{\text{sub}\}$'s boyfriend? & Who is Monica's boyfriend? \\ \cline{2-4}
 & ex-husband  & Who is $\{\text{sub}\}$'s ex-husband? & Who is Carol's ex-husband? \\ \cline{2-4}
 & ex-wife  & Who is $\{\text{sub}\}$'s ex-wife? & Who is Ross's ex-wife? \\ \cline{2-4}
 & ex-girlfriend  & Who is $\{\text{sub}\}$'s ex-girlfriend? & Who is Ross's ex-girlfriend? \\ \cline{2-4}
 & ex-boyfriend  & Who is $\{\text{sub}\}$'s ex-boyfriend? & Who is Rachel's ex-boyfriend? \\ \cline{2-4}
 & brother  & Who is $\{\text{sub}\}$'s brother? & Who is Monica's brother? \\ \cline{2-4}
 & sister & Who is $\{\text{sub}\}$'s sister? & Who is Ross's sister? \\ \hline
\end{tabular}%
\vspace{-10mm}
}
\caption{Templates for one-hop questions without temporal information.
\label{app:question_onehop_without_time_templates}
}
\end{table*}

\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\hline
\textbf{Question Type} & \textbf{Relation} &\textbf{Template} & \textbf{Question Example}\\ \hline
\multirow{16}{*}{\textbf{With Time}} & boss & Who was $\{\text{sub}\}$'s boss on $\{\text{time}\}$? & Who was Chandler's boss on September 26th, 1994? \\ \cline{2-4} 
 & client & Who was $\{\text{sub}\}$'s client on $\{\text{time}\}$? & Who was Chandler's client on September 26th, 1994? \\ \cline{2-4} 
 & neighbor & Who was $\{\text{sub}\}$'s neighbor on $\{\text{time}\}$? & Who was Chandler's neighbor on September 26th, 1994? \\ \cline{2-4} 
 & roommate & Who was $\{\text{sub}\}$'s roommate on $\{\text{time}\}$? & Who was Chandler's roommate on September 26th, 1994? \\ \cline{2-4} 
 & fiance  & Who was $\{\text{sub}\}$'s fiance on $\{\text{time}\}$? & Who was Rachel's fiance on September 26th, 1994? \\ \cline{2-4} 
 & fiancee  & Who was $\{\text{sub}\}$'s fiancee on $\{\text{time}\}$? & Who was Ross's fiancee on September 26th, 1994? \\ \cline{2-4} 
 & pet  & Who was $\{\text{sub}\}$'s pet on $\{\text{time}\}$? & Who was Ross's pet on September 26th, 1994? \\ \cline{2-4} 
 & dating with  & Who dated $\{\text{sub}\}$ on $\{\text{time}\}$? & Who dated Ross on September 26th, 1994? \\ \cline{2-4} 
 & job  & What was $\{\text{sub}\}$'s job on $\{\text{time}\}$? & What was Monica's job on September 26th, 1994? \\ \cline{2-4} 
 & place of work  & Where did $\{\text{sub}\}$ work on $\{\text{time}\}$? & Where did Monica work on September 26th, 1994? \\ \cline{2-4} 
 & age  & How old was $\{\text{sub}\}$ on $\{\text{time}\}$? & How old was Monica on September 26th, 1994? \\ \cline{2-4} 
 & major  & What was $\{\text{sub}\}$'s major on $\{\text{time}\}$? & What was Ross's major on September 26th, 1994? \\ \cline{2-4} 
 & husband  & Who was $\{\text{sub}\}$'s husband on $\{\text{time}\}$? & Who was Emily's husband on September 26th, 1994? \\ \cline{2-4}
 & wife  & Who was $\{\text{sub}\}$'s wife on $\{\text{time}\}$? & Who was Ross's wife on September 26th, 1994? \\ \cline{2-4}
 & girlfriend  & Who was $\{\text{sub}\}$'s girlfriend on $\{\text{time}\}$? & Who was Ross's girlfriend on September 26th, 1994? \\ \cline{2-4}
 & boyfriend  & Who was $\{\text{sub}\}$'s boyfriend on $\{\text{time}\}$? & Who was Rachel's boyfriend on September 26th, 1994? \\ \hline
\end{tabular}%
}
\caption{Templates for one-hop questions with temporal information.
\label{app:question_onehop_time_templates}
}
\end{table*}

\begin{table*}[h]
\vspace{2mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\hline
\textbf{First Relation} & \textbf{Second Relation} & \textbf{Template} & \textbf{Question Example} \\ \hline
\multirow{17}{*}{\begin{tabular}[c]{@{}l@{}}roommate, wife, husband, \\ girlfriend, boyfriend, client, \\ neighbor, boss, subordinate, \\ fiance, fiancee\end{tabular}} & \begin{tabular}[c]{@{}l@{}}roommate, wife, husband, pet,\\ girlfriend, boyfriend, client, neighbor,\\ boss, subordinate, fiance, fiancee\end{tabular} & \begin{tabular}[c]{@{}l@{}}\{sub1\} had a \{First Relation\} on \{time1\}. \\ Who was the \{Second Relation\} of the \\ \{First Relation\} on \{time2\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica had a roommate on September 26th, 1994.\\ Who was the boyfriend of the roommate \\ on October 5th, 1996?\end{tabular} \\ \cline{2-4} 
 & dating with & \begin{tabular}[c]{@{}l@{}}\{sub1\} had a \{First Relation\} on \{time1\}. \\ Who dated the \{First Relation\} on \{time2\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica had a roommate on September 26th, 1994. \\ Who dated the roommate on October 5th, 1996?\end{tabular} \\ \cline{2-4} 
 & job, major, age & \begin{tabular}[c]{@{}l@{}}\{sub1\} had a \{First Relation\} on \{time1\}. \\ What was the \{Second Relation\} of the\\ \{First Relation\} on \{time2\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica had a roommate on September 26th, 1994.\\ What was the job of the roommate \\ on October 5th, 1996?\end{tabular} \\ \cline{2-4} 
 & \begin{tabular}[c]{@{}l@{}}mother, father, son, daughter, \\ sister, brother\end{tabular} & \begin{tabular}[c]{@{}l@{}}\{sub1\} had a \{First Relation\} on \{time1\}. \\ Who is the \{Second Relation\} of the\\ \{First Relation\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica had a roommate on September 26th, 1994.\\ Who is the mother of the roommate?\end{tabular} \\ \cline{2-4} 
 & date of birth, place of birth, & \begin{tabular}[c]{@{}l@{}}\{sub1\} had a \{First Relation\} on \{time1\}. \\ When (Where) was the \{First Relation\} born?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica had a roommate on September 26th 1994. \\ When was the roommate born?\end{tabular} \\ \cline{2-4} 
 & place of work & \begin{tabular}[c]{@{}l@{}}\{sub1\} had a \{First Relation\} on \{time1\}. \\ Where did the \{First Relation\} work \\ on \{time2\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica had a roommate on September 26th, 1994. \\ Where did the roommate work \\ on October 5th, 1996?\end{tabular} \\ \cline{2-4} 
 & hometown & \begin{tabular}[c]{@{}l@{}}\{sub1\} had a \{First Relation\} on \{time1\}.\\ Where is the hometown of the \\ \{First Relation\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica had a roommate on September 26th, 1994.\\ Where is the hometown of the roommate?\end{tabular} \\ \hline
dating with & \begin{tabular}[c]{@{}l@{}}roommate, wife, husband, \\ girlfriend, boyfriend, client, neighbor,\\ boss, subordinate, fiance, fiancee\end{tabular} & \begin{tabular}[c]{@{}l@{}}\{sub1\} dated a person on \{time1\}. \\ Who was the \{Second Relation\} of the \\ person on \{time2\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Monica dated a person on September 26th, 1994.\\ Who was the boss of the person \\ on October 5th, 1996?\end{tabular} \\ \hline
\multirow{13}{*}{\begin{tabular}[c]{@{}l@{}}mother, father, son, \\ daughter, sister, brother\end{tabular}} & \begin{tabular}[c]{@{}l@{}}roommate, wife, husband, \\ girlfriend, boyfriend, client, neighbor, \\ boss, subordinate, fiance, fiancee\end{tabular} & \begin{tabular}[c]{@{}l@{}}Who was the \{Second Relation\} of \{sub1\}'s \\ \{First Relation\} on \{time2\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Who was the roommate of Ross's \\ sister on September 26th, 1994?\end{tabular} \\ \cline{2-4} 
  & dating with & \begin{tabular}[c]{@{}l@{}}Who dated \{sub1\}'s \{First Relation\} \\ on \{time2\}?\end{tabular} & Who dated Ben's father on September 26th, 1994? \\ \cline{2-4} 
 & job, age, major & \begin{tabular}[c]{@{}l@{}}What was the \{Second Relation\} of \\ \{sub1\}'s \{First Relation\} on \{time2\}?\end{tabular} & What was the job of Ben's father on September 26th, 1994? \\\cline{2-4} 
  & \begin{tabular}[c]{@{}l@{}}mother, father, son, daughter, \\ sister, brother\end{tabular} & \begin{tabular}[c]{@{}l@{}}Who is the \{Second Relation\} of \\ \{sub1\}'s \{First Relation\}?\end{tabular} & Who is the mother of Ross's son? \\ \cline{2-4} 
 & date of birth, place of birth & \begin{tabular}[c]{@{}l@{}}When (Where) was \{sub1\}'s \{First Relation\} \\ born?\end{tabular} & When was Monica's brother born? \\ \cline{2-4} 
 & place of work & \begin{tabular}[c]{@{}l@{}}Where did \{sub1\}'s \{First Relation\} \\ work on \{time2\}?\end{tabular} & \begin{tabular}[c]{@{}l@{}}Where did Monica's brother work \\ on October 5th, 1996?\end{tabular} \\ \cline{2-4} 
 & hometown & \begin{tabular}[c]{@{}l@{}}Where is the hometown of \\ \{sub1\}'s \{First Relation\}?\end{tabular} & Where is the hometown of Ross's son? \\ 
 \hline
\end{tabular}%
\vspace{-6mm}
}
\caption{Templates for two-hop questions.
\label{app:question_twohop_templates}
}
\end{table*}


==> tabs/app_style_transfer_example.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
\textbf{Original Question} & \textbf{Character} & \textbf{Style Transferred Question} \\ \hline
\multirow{9}{*}{By the way, how did Rachel buy her new boots?} & Default & \begin{tabular}[c]{@{}l@{}}Hey, any idea what Rachel used to snag those stylish \\ new boots of hers?\end{tabular} \\ \cline{2-3} 
 & Monica & \begin{tabular}[c]{@{}l@{}}Hey, do you know what Rachel used to snag those super \\ cute new boots she's been rocking?\end{tabular} \\ \cline{2-3} 
 & Chandler & \begin{tabular}[c]{@{}l@{}}So, could we BE any more curious about how Rachel \\ snagged those new boots?\end{tabular} \\ \cline{2-3} 
 & Joey & \begin{tabular}[c]{@{}l@{}}Hey, how did Rachel manage to snag those killer \\ boots, huh?\end{tabular} \\ \cline{2-3} 
 & Phoebe & \begin{tabular}[c]{@{}l@{}}Oh my gosh! Do you have any idea how Rachel snagged\\  those super cute new boots?\end{tabular} \\  \hline
\multirow{9}{*}{By the way, who dated Monica on September 22, 1994?} & Default & \begin{tabular}[c]{@{}l@{}}So, who was Monica's date on the night of \\ September 22, 1994?\end{tabular} \\ \cline{2-3} 
 & Chandler & \begin{tabular}[c]{@{}l@{}}Oh, could you BE any more specific about who was \\ going out with Monica on September 22, 1994?\end{tabular} \\ \cline{2-3} 
 & Joey & \begin{tabular}[c]{@{}l@{}}Hey, just outta curiosity, who was goin' out with \\ Monica on September 22, 1994?\end{tabular} \\ \cline{2-3} 
 & Phoebe & \begin{tabular}[c]{@{}l@{}}Oh my gosh, so like, who was Monica's date on that \\ super specific day, September 22, 1994?\end{tabular} \\ \cline{2-3} 
 & Rachel & \begin{tabular}[c]{@{}l@{}}Oh my god, so like, who was going out with Monica \\ on September 22, 1994?'\end{tabular} \\ \hline
\multirow{14}{*}{\begin{tabular}[c]{@{}l@{}}By the way, Rachel had a roommate on October 28, 1994. \\ Who dated the roommate in September 1994?\end{tabular}} & Default & \begin{tabular}[c]{@{}l@{}}Oh. My. God. Remember when Rachel had a roommate \\ back on October 28, 1994? So, who was going out with\\  that roommate by September 1994?\end{tabular} \\ \cline{2-3} 
 & Monica & \begin{tabular}[c]{@{}l@{}}Hey, just out of curiosity, do you know who was going \\ out with Rachel's roommate from back in September 1994? \\ I remember she got that roommate around October 28, 1994.\end{tabular} \\ \cline{2-3} 
 & Chandler & \begin{tabular}[c]{@{}l@{}}So, just for a little stroll down memory lane, Rachel \\ was bunking with someone on October 28, 1994. \\ Any wild guesses on who was dating this mystery \\ co-habitant by September 1994?\end{tabular} \\ \cline{2-3} 
 & Joey & \begin{tabular}[c]{@{}l@{}}Hey, so you know how Rachel was living with someone\\  back on October 28, 1994, right? So I'm just wonderin' \\ here, who was going out with this roommate of hers in \\ September 1994?\end{tabular} \\ \cline{2-3} 
 & Phoebe & \begin{tabular}[c]{@{}l@{}}By the way, Rachel had a roommate on October 28, 1994. \\ Who dated the roommate in September 1994?\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Examples of the results of character style transfer.
\label{app:question_styletransfer}
}
\end{table*}

==> tabs/bigbang_original_6s.tex <==
\begin{table*}[h]
\centering
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width % \multicolumn{1}{p{2cm}}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c l c c c c c c c} 
\toprule % \multirow{2}[7]{*}{\textbf{Model}}
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
\multirow{3}{*}{API} & GPT-4o-mini & 22.68 (2.12)$^\dagger$ & 19.77 (2.02) & \textbf{36.63 (1.82)} & 30.10 (1.44) & 29.54 (0.71) & 32.34 (0.58) & 35.72 (0.81) \\
& GPT-3.5 & \textbf{32.49 (1.72)} & 25.32 (1.20) & 35.59 (2.12) & 33.86 (1.09) & 27.81 (0.40) & 32.97 (0.86) & \textbf{37.02 (1.13)}\\
 & Gemini 1.0 pro & 3.49 (0.69) & 25.87 (1.23) & 30.72 (0.18) & \textbf{38.16 (1.25)} & \textbf{37.42 (0.68)} & 32.09 (0.44) & 36.30 (0.32) \\
 \midrule
\multirow{9}{*}{Open} & \textsc{Tülu} 2-70B & 0.62 (0.13) & 21.08 (0.70) & 18.95 (1.07) & 22.36 (0.65) & 34.64 (0.69) & 9.08 (1.00) & 20.22 (1.48) \\
 & \textsc{Tülu} 2-7B & 0.53 (0.18) & 15.58 (1.34) & 22.26 (0.53) & 29.99 (0.57) & 16.84 (2.13) & 21.48 (0.77) & 28.69 (1.15) \\
 & Llama3.1-70B & 0.25 (0.07)$^\dagger$ & 21.55 (0.93) & 0.15 (0.12) & 1.26 (0.31) & 34.21 (1.59) & 3.89 (1.05) & 14.89 (1.74) \\
 & Llama3.1-8B & 21.30 (1.68)$^\dagger$ & 12.80 (1.06) & 25.50 (0.16) & 18.56 (0.99) & 23.10 (2.69) & 25.48 (3.65) & 20.75 (1.58) \\
 & Mixtral-8x7B & 1.95 (0.34) & 15.91 (0.71) & 34.52 (1.12) & 16.83 (1.60) & 17.45 (0.49) & \textbf{34.98 (0.99)} & 13.83 (2.18) \\
 & Mistral-7B & 3.11 (0.21) & 24.69 (1.82) & 34.26 (0.60) & 32.17 (1.39) & 30.23 (0.62) & 33.36 (0.56) & 29.19 (1.54) \\
 & Gemma-7B & 16.40 (0.74) & 21.40 (2.33) & 19.74 (2.45) & 16.67 (0.40) & 24.50 (1.87) & 20.22 (1.39) & 16.12 (0.52) \\
 & Gemma-2B & 1.56 (0.06) & \textbf{28.94 (0.35)} & 26.12 (2.22) & 33.47 (1.41) & 27.92 (0.68) & 29.40 (1.79) & 34.86 (3.20) \\
\bottomrule
\vspace{-4mm}
\end{tabular}
\end{adjustbox}
% \vspace{-5mm}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\caption{The performances of the agents on The Big Bang Theory dialogue in \simname (time limit = 6 seconds). We conducted experiments three times and reported the accuracies and the standard deviations.
\label{bigbangres}}
\end{table*}


==> tabs/friends_new_name_6s.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.1}
\centering
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width % \multicolumn{1}{p{2cm}}
\begin{tabular}{c l c c c c c c c} 
\toprule % \multirow{2}[7]{*}{\textbf{Model}}
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
API & GPT-4o-mini & \textbf{31.72 (1.69)}$^\dagger$ & 29.29 (0.74) & \textbf{42.95 (2.04)} & \textbf{31.12 (0.94)} & 35.08 (1.02) & \textbf{38.14 (3.63)} & \textbf{36.91 (2.00)} \\
\midrule
\multirow{8}{*}{Open} & \textsc{Tülu} 2-70B & 0.21 (0.07) & 18.24 (0.84) & 20.60 (1.00) & 18.64 (1.81) & 31.71 (2.22) & 7.82 (1.57) & 17.31 (0.61)\\
 & \textsc{Tülu} 2-7B & 0.74 (0.15) & 13.19 (0.35) & 19.54 (1.29) & 26.07 (2.00) & 13.87 (0.71) & 18.35 (1.21) & 27.48 (2.04)\\
 & Llama3.1-70B & 0.64 (0.10)$^\dagger$ & \textbf{29.29 (0.59)} & 0.60 (0.12) & 15.07 (5.12) & \textbf{39.08 (0.99)} & 2.43 (0.10) & 18.18 (0.16) \\
 & Llama3.1-8B & 26.61 (1.24)$^\dagger$ & 26.86 (0.78) & 31.20 (1.87) & 27.08 (0.63) & 24.82 (1.07) & 31.72 (1.66) & 22.69 (0.63) \\
 & Mixtral-8x7B & 2.41 (0.40) & 14.90 (0.82) & 23.55 (0.40) & 15.64 (0.47) & 16.43 (1.68) & 22.95 (0.68) & 13.22 (1.61) \\
 & Mistral-7B & 3.35 (0.58) & 24.44 (1.13) & 31.39 (0.70) & 24.26 (1.60) & 29.82 (0.95) & 30.21 (0.90) & 23.90 (0.51) \\
 & Gemma-7B & 18.05 (0.97) & 22.52 (0.81) & 20.64 (0.26) & 16.63 (1.59) & 23.41 (1.26) & 18.34 (0.82) & 19.48 (2.45) \\
 & Gemma-2B & 0.47 (0.13) & 24.31 (0.96) & 24.77 (0.74) & 25.74 (1.46) & 28.41 (1.20) & 24.68 (1.45) & 24.75 (1.50) \\
\bottomrule
\vspace{-4mm}
\end{tabular}
\end{adjustbox}
% \vspace{-5mm}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\caption{The performances of the agents on Friends dialogue in \simname (time limit = 6 seconds, with new names replaced). We conducted experiments three times and reported the accuracies and the standard deviations.}
\label{newname6s}
\end{table*}

==> tabs/friends_new_name_infinite.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.1}
\centering
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width % \multicolumn{1}{p{2cm}}
\begin{tabular}{c l c c c c c c c} 
\toprule % \multirow{2}[7]{*}{\textbf{Model}}
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
API & GPT-4o-mini & 32.06 (0.52)$^\dagger$ & 30.01 (1.09) & \textbf{46.57 (1.56)} & 34.44 (1.53) & 34.23 (0.99) & 38.78 (0.24) & 37.97 (1.24) \\
\midrule
\multirow{8}{*}{Open} & \textsc{Tülu} 2-70B & 2.17 (0.46) & 27.24 (1.17) & 33.34 (1.17) & 32.85 (1.85) & 34.95 (0.47) & 29.41 (1.22) & 33.55 (2.79)\\
 & \textsc{Tülu} 2-7B & 0.63 (0.26) & \textbf{30.26 (1.03)} & 27.68 (1.24) & 30.98 (1.08) & 30.99 (0.22) & 27.93 (1.97) & 31.80 (2.05)\\
 & Llama3.1-70B & 31.03 (1.91)$^\dagger$ & 28.91 (2.33) & 38.44 (5.98) & \textbf{41.68 (3.68)} & \textbf{38.40 (1.10)} & \textbf{40.83 (1.07)} & \textbf{44.27 (0.57)} \\
 & Llama3.1-8B & 26.65 (1.19)$^\dagger$ & 25.80 (0.18) & 32.01 (1.10) & 30.48 (1.30) & 29.50 (1.10) & 32.82 (0.63) & 32.23 (2.32) \\
 & Mixtral-8x7B & \textbf{38.92 (1.61)} & 26.91 (1.46) & 39.98 (2.98) & 27.02 (0.42) & 30.27 (1.37) & 35.89 (0.37) & 29.52 (1.28) \\
 & Mistral-7B & 29.10 (1.34) & 23.33 (0.83) & 34.59 (0.80) & 27.87 (2.66) & 30.59 (2.09) & 30.45 (0.89) & 27.93 (0.99) \\
 & Gemma-7B & 17.37 (0.77) & 22.58 (1.62) & 21.41 (1.53) & 21.61 (1.53) & 23.90 (0.90) & 21.61 (1.09) & 20.88 (0.91)\\
 & Gemma-2B & 0.37 (0.07) & 23.48 (1.85) & 23.13 (1.14) & 25.72 (2.67) & 29.12 (1.90) & 24.88 (1.40) & 24.81 (1.31)\\
\bottomrule
\vspace{-4mm}
\end{tabular}
\end{adjustbox}
% \vspace{-5mm}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\caption{The performances of the agents on Friends dialogue in \simname (without a time limit and with new names replaced). We conducted experiments three times and reported the accuracies and the standard deviations.}
\label{newnameinfinite}
\end{table*}

==> tabs/friends_original_6s.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}m{3cm}}
\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}
\centering
\begin{adjustbox}{max width=\linewidth} 
\begin{tabular}{c l c c c c c c c} 
\toprule 
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
\multirow{3}{*}{API} & GPT-4o-mini & \textbf{38.53 (0.89)}$^\dagger$ & \textbf{32.65 (2.65)} & \textbf{49.04 (1.67)} & \textbf{40.27 (1.36)} & \textbf{40.10 (0.75)} & \textbf{44.36 (2.36)} & \textbf{42.53 (1.26)} \\
& GPT-3.5 & 31.82 (1.31) &  25.58 (1.78) & 39.70 (1.86) & 32.09 (0.84) & 32.06 (1.60) & 36.84 (1.77) & 36.69 (1.25) \\
& Gemini 1.0 pro & 2.96 (0.31) & 28.77 (1.83) & 25.07 (2.40) & 35.27 (1.80) & 34.22 (0.49) & 31.83 (0.41) & 35.75 (2.93) \\
 
 \midrule
\multirow{8}{*}{Open} & \textsc{Tülu} 2-70B & 0.37 (0.15) & 20.94 (0.75) & 20.27 (0.99) & 19.75 (0.08) & 31.76 (1.84) & 10.15 (0.55) & 18.87 (0.30)\\
 & \textsc{Tülu} 2-7B & 0.84 (0.15) & 12.68 (0.24) & 19.58 (1.04) & 26.84 (0.85) & 14.08 (0.89) & 17.39 (1.37) & 25.21 (1.28)\\
 & Llama3.1-70B & 0.60 (0.06)$^\dagger$ & 31.08 (1.21) & 0.55 (0.12) & 16.26 (5.05) & 39.00 (0.30) & 2.26 (0.42) & 20.14 (0.22) \\
 & Llama3.1-8B & 28.82 (1.94)$^\dagger$ & 27.12 (0.95) & 34.14 (0.85) & 30.91 (0.63) & 29.76 (1.31) & 33.25 (0.57) & 24.48 (0.60) \\
 & Mixtral-8x7B & 1.88 (0.26) & 16.84 (0.95) & 26.23 (0.90) & 17.11 (1.94) & 17.94 (1.32) & 26.78 (1.04) & 15.40 (1.39) \\
 & Mistral-7B & 2.82 (0.46) & 24.22 (2.04) & 33.07 (1.01) & 29.29 (1.76) & 28.30 (1.93) & 29.15 (1.67) & 25.41 (1.53) \\
 & Gemma-7B & 16.60 (0.84) & 22.11 (1.73) & 24.30 (2.04) & 18.33 (1.37) & 26.42 (2.48) & 22.54 (0.78) & 18.80 (0.64) \\
 & Gemma-2B & 0.68 (0.20) & 24.06 (2.03) & 24.22 (1.34) & 25.79 (1.00) & 25.31 (1.55) & 24.48 (1.62) & 25.78 (1.12)\\
\hline
& Random Guessing & 20.00 & 20.00 & 20.00 & 20.00 & 20.00 & 20.00 & 20.00\\
% \multicolumn{2}{l}{Random Guessing} & 20.00 & 20.00 & 20.00 & 20.00 & 20.00 & 20.00 & 20.00 \\
\bottomrule
\vspace{-5mm}
\end{tabular}
\end{adjustbox}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\vspace{-4mm}
\caption{The performance of the agents on Friends dialogue in \simname (time limit = 6 seconds). We conducted experiments three times and reported the accuracy and standard deviations. \textbf{Bold} indicates the highest performance for each retrieval method.}
\vspace{-6mm}
\label{mainres}
\end{table*}



==> tabs/friends_original_infinite.tex <==



% \newcolumntype{C}{>{\centering\arraybackslash}m{3cm}}
% \begin{table}[t]
% \renewcommand{\arraystretch}{1.1}
% \centering
% % \vspace{-3mm}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{l c c c c} 
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Base LLM}} & \multicolumn{1}{c}{\textbf{BM25}} & \multicolumn{1}{c}{\textbf{OpenAI Embedding}} \\
% \cmidrule(lr){3-3} \cmidrule(lr){4-4}
%  & & \textbf{Session Entire} & \textbf{Session Sum.} \\
% \midrule
% GPT-4o-mini & 38.91 (0.99)$^\dagger$ & \textbf{49.21 (0.12)} & 42.40 (0.99) \\
% Llama3.1-70B & 36.36 (0.68)$^\dagger$ & 43.17 (0.99) & \textbf{48.49 (0.97)} \\
% Llama3.1-8B & 28.78 (0.34)$^\dagger$ & 34.70 (1.75) & 35.59 (1.09) \\
% Mixtral-8x7B & \textbf{42.19 (1.76)} & 46.47 (1.75) & 34.18 (0.96) \\
% Mistral-7B & 32.93 (0.59) & 35.09 (1.76) & 30.80 (1.75) \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \tiny{\makebox[\linewidth][r]{$\dagger$: Limited the maximum context length to 8k tokens.}}
% \vspace{-4mm}
% \caption{The performance of the top-performing agents on Friends in \simname \textbf{without time limit}. The full experimental results are provided in Appendix X.}
% \vspace{-2mm}
% \label{friendsinfinite}
% \end{table}

% \newcommand{\uli}[1]{\underline{#1}}

% \newcolumntype{C}{>{\centering\arraybackslash}m{3cm}}
% \begin{table}[t]
% \renewcommand{\arraystretch}{1.1}
% \centering
% % \vspace{-3mm}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{l c cc cc} 
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Base LLM}} & \multicolumn{2}{c}{\textbf{BM25}} & \multicolumn{2}{c}{\textbf{OpenAI}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
%  & & \textbf{SE} & \textbf{SS} & \textbf{SE} & \textbf{SS} \\
% \midrule
% GPT-4o-mini & 38.91$^\dagger$ & \uli{\textbf{49.21}}& 42.23 & \textbf{43.64} & 42.40 \\
% GPT-3.5 & 31.81 & \uli{39.45} & 32.77 & 35.78 & 35.98 \\
% Gemini 1.0 pro & 28.36 & \uli{39.90} & 34.11 & 30.93 & 33.96 \\
% \hline
% Llama3.1-70B & 36.36$^\dagger$ & 43.17 & \textbf{43.81} & 43.17 & \uli{\textbf{48.49}} \\
% Llama3.1-8B & 28.78$^\dagger$ & 34.70 & 33.93 & 32.91 & \uli{35.59} \\
% Mixtral-8x7B & \textbf{42.19} & \uli{46.47} & 32.31 & 41.24 & 34.18 \\
% Mistral-7B & 32.93 & \uli{35.09} & 30.16 & 31.00 & 30.10 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \tiny{\makebox[\linewidth][r]{$\dagger$: Limited the maximum context length to 8k tokens.}}
% \vspace{-4mm}
% \caption{The performance of the top-performing agents on Friends in \simname \textbf{without time limit}. \textbf{SE} and \textbf{SS} denote Session Entire and Session Summary, respectively. \textbf{Bold} indicates the highest performance for each retrieval method, and \uli{underlined values} indicate the best-performing retrieval method for each model. The full experimental results are in Appendix X.}
% \vspace{-2mm}
% \label{friendsinfinite}
% \end{table}

\newcommand{\uli}[1]{\underline{#1}}

\newcolumntype{C}{>{\centering\arraybackslash}m{3cm}}
\begin{table}[t]
\renewcommand{\arraystretch}{1.1}
\centering
% \vspace{-3mm}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{l c ccc ccc} 
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\makecell[c]{\textbf{Base} \\ \textbf{LLM}}} & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
 & & \textbf{UT} & \textbf{SE} & \textbf{SS} & \textbf{UT} & \textbf{SE} & \textbf{SS} \\
\midrule
GPT-4o-mini & 38.91$^\dagger$ & \textbf{34.44} & \uli{\textbf{49.21}} & 42.23 & 38.91 & \textbf{43.64} & 42.40 \\
GPT-3.5 & 31.81 & 26.91 & \uli{39.45} & 32.77 & 32.41 & 35.78 & 35.98 \\
Gemini 1.0 pro & 28.36 & 28.10 & \uli{39.90} & 34.11 & 34.26 & 30.93 & 33.96 \\
\hline
Llama3.1-70B & 36.36$^\dagger$ & 31.84 & 43.17 & \textbf{43.81} & \textbf{39.85} & 43.17 & \uli{\textbf{48.49}} \\
Llama3.1-8B & 28.78$^\dagger$ & 29.89 & 34.70 & 33.93 & 31.63 & 32.91 & \uli{35.59} \\
Mixtral-8x7B & \textbf{42.19} & 31.84 & \uli{46.47} & 32.31 & 35.51 & 41.24 & 34.18 \\
Mistral-7B & 32.93 & 28.20 & \uli{35.09} & 30.16 & 30.12 & 31.00 & 30.10 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\tiny{\makebox[\linewidth][r]{$\dagger$: Limited the maximum context length to 8k tokens.}}
\vspace{-4mm}
\caption{The performance of the top-performing agents on Friends in \simname \textbf{without time limit}. \textbf{UT}, \textbf{SE}, and \textbf{SS} denote Utterance, Session Entire, and Session Summary, respectively. \textbf{Bold} indicates the highest performance for each retrieval method, and \uli{underlined values} indicate the best-performing retrieval method for each model. The full experimental results are in Appendix~\ref{unlimitedres}.}
% \vspace{-2mm}
\label{friendsinfinite}
\end{table}


==> tabs/friends_original_infinite_with_oracle.tex <==
\begin{table}[t]
\centering
\caption{friends orignal infinite with oracle}
%\small % Reduce font size
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width
\begin{tabular}{c c c c c c c c c c}
\toprule
\multirow{2}[7]{*}{\textbf{Type}} & \multirow{2}[7]{*}{\textbf{Model}} & \multirow{2}[7]{*}{\textbf{No Retrieval}} & \multicolumn{6}{c}{\textbf{RAG based}} \\
\cmidrule(lr){4-10}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}} & \multicolumn{1}{c}{\textbf{Oracle}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-10}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum} & \textbf{Session Entire}\\
\midrule
\multirow{2}{*}{API} & GPT-3.5 & 31.81 (1.33) & 26.91 (2.3) & 39.45 (1.4) & 32.77 (1.31) & 32.41 (0.96) & 35.78 (0.74) & 35.98 (1.75) & 51.05 (1.94)\\
 & Gemini 1.0 pro & 28.36 (0.97) & 28.1 (1.08) & 39.9 (1.08) & 34.11 (1.64) & 34.26 (2.91) & 30.93 (2.17) & 33.96 (2.11) & 49.17 (6.54)\\
 \midrule
\multirow{9}{*}{Open} & Tulu2-70B & 3.31 (0.32) & 29.87 (0.65) & 35.87 (2.56) & 34.72 (1.63) & 37.07 (0.72) & 33.63 (1.32) & \textbf{38.62 (1.94)} & 55.12 (1.10)\\
 & Tulu2-7B & 1.57 (0.12) & 28.93 (2.81) & 28.72 (1.8) & 30.86 (2.29) & 34.55 (0.47) & 31.04 (0.96) & 32.12 (0.75) & 46.93 (0.88)\\
 & LLaMA2-70B-chat & 35.55 (2.06) & \textbf{33.67 (0.58)} & 35.62 (1.74) & \textbf{35.71 (1.87)} & \textbf{38.8 (0.98)} & 34.92 (1.62) & 37.45 (1.98) & 54.26 (1.43)\\
 & LLaMA2-7B-chat & 21.8 (1.02) & 25.29 (1.34) & 27.47 (1.92) & 23.31 (1.22) & 29.34 (1.79) & 25.58 (2.47) & 24.22 (1.4) & 39.70 (1.82)\\
 & Mixtral & \textbf{42.19 (1.76)} & 31.84 (0.78) & \textbf{46.47 (1.75)} & 32.31 (1.09) & 35.51 (0.19) & \textbf{41.24 (2.9)} & 34.18 (0.96) & 62.72 (1.45)\\
 & Mistral-7B & 32.93 (0.59) & 28.2 (1.17) & 35.09 (1.76) & 30.16 (1.82) & 30.12 (1.45) & 31.0 (1.93) & 30.8 (1.75) & 53.42 (0.86)\\
 & Gemma-7B & 18.78 (0.87) & 22.26 (1.52) & 23.62 (2.09) & 19.83 (1.74) & 25.07 (0.49) & 22.48 (0.25) & 20.08 (0.76) & 22.68 (0.40)\\
 & Gemma-2B & 1.16 (0.26) & 25.03 (1.54) & 24.64 (1.31) & 24.84 (2.05) & 28.06 (1.38) & 24.56 (2.6) & 28.28 (1.94) & 26.85 (0.84)\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{friendsinfinitewithoracle}
\end{table}


==> tabs/friends_original_with_oracle_6s.tex <==
\begin{table}[ht]
\centering
\caption{friends original with oracle 6s}
\label{friends_original_with_oracle_6s}
%\small % Reduce font size
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width
\begin{tabular}{c c c c c c c c c c}
\toprule
\multirow{2}[7]{*}{\textbf{Type}} & \multirow{2}[7]{*}{\textbf{Model}} & \multirow{2}[7]{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG based}} \\
\cmidrule(lr){4-10}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}} & \multicolumn{1}{c}{\textbf{Oracle}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-10}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum} & \textbf{Session Entire}\\
\midrule
\multirow{2}{*}{API} & GPT-3.5 & \textbf{31.82 (1.31)} &  25.58 (1.78) & \textbf{39.7 (1.86)} & 32.09 (0.84) & 32.06 (1.6) & \textbf{36.84 (1.77)} & \textbf{36.69 (1.25)} & 51.05 (1.94)\\
 & Gemini 1.0 pro & 2.96 (0.31) & \textbf{28.77 (1.83)} & 25.07 (2.4) & \textbf{35.27 (1.8)} & \textbf{34.22 (0.49)} & 31.83 (0.41) & 35.75 (2.93) & 49.17 (6.54)\\
 \midrule
\multirow{9}{*}{Open} & Tulu2-70B & 0.37 (0.15) & 20.94 (0.75) & 20.27 (0.99) & 19.75 (0.08) & 31.76 (1.84) & 10.15 (0.55) & 18.87 (0.3) & 55.12 (1.10)\\
 & Tulu2-7B & 0.84 (0.15) & 12.68 (0.24) & 19.58 (1.04) & 26.84 (0.85) & 14.08 (0.89) & 17.39 (1.37) & 25.21 (1.28) & 46.93 (0.88)\\
 & Llama2-7B & 0.05 (0.08) & 0.0 (0.0) & 1.26 (0.77) & 0.21 (0.08) & 0.0 (0.0) & 0.16 (0.0) & 0.05 (0.08) & 54.26 (1.43)\\
 & Llama2-7B & 22.01 (1.5) & 22.63 (1.61) & 23.14 (1.17) & 19.24 (0.51) & 25.41 (1.38) & 21.22 (1.44) & 19.23 (1.32) & 39.70 (1.82)\\
 & Mixtral-8x7B & 1.88 (0.26) & 16.84 (0.95) & 26.23 (0.9) & 17.11 (1.94) & 17.94 (1.32) & 26.78 (1.04) & 15.4 (1.39) & 62.72 (1.45)\\
 & Mistral-7B & 2.82 (0.46) & 24.22 (2.04) & 33.07 (1.01) & 29.29 (1.76) & 28.3 (1.93) & 29.15 (1.67) & 25.41 (1.53) & 53.42 (0.86)\\
 & Gemma-7B & 16.6 (0.84) & 22.11 (1.73) & 24.3 (2.04) & 18.33 (1.37) & 26.42 (2.48) & 22.54 (0.78) & 18.8 (0.64) & 22.68 (0.40)\\
 & Gemma-2B & 0.68 (0.2) & 24.06 (2.03) & 24.22 (1.34) & 25.79 (1.0) & 25.31 (1.55) & 24.48 (1.62) & 25.78 (1.12) & 26.85 (0.84)\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tabs/friends_shuffle_6s.tex <==
\begin{table*}[h]
\centering
%\small % Reduce font size
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width % \multicolumn{1}{p{2cm}}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c l c c c c c c c} 
\toprule % \multirow{2}[7]{*}{\textbf{Model}}
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
API & GPT-4o-mini & \textbf{31.37 (1.57)}$^\dagger$ & 27.54 (1.85) & \textbf{40.36 (0.73)} & \textbf{29.71 (0.84)} & 33.63 (0.30) & \textbf{35.93 (1.56)} & \textbf{37.30 (1.71)} \\
\midrule
\multirow{8}{*}{Open} & \textsc{Tülu} 2-70B & 0.31 (0.13) & 17.03 (0.94) & 15.20 (0.87) & 18.45 (1.04) & 26.89 (0.54) & 6.92 (0.47) & 12.86 (1.23) \\
 & \textsc{Tülu} 2-7B & 0.73 (0.29) & 12.50 (1.73) & 17.58 (1.14) & 24.21 (1.09) & 10.20 (0.21) & 14.26 (0.92) & 21.03 (0.58) \\
 & Llama3.1-70B & 0.51 (0.00)$^\dagger$ & \textbf{27.84 (1.89)} & 0.60 (0.06) & 13.84 (2.31) & \textbf{35.67 (1.89)} & 1.53 (028) & 20.90 (0.37) \\
 & Llama3.1-8B & 25.84 (1.16)$^\dagger$ & 25.24 (0.30) & 28.86 (1.01) & 24.56 (0.99) & 28.86 (1.10) & 32.35 (1.51) & 24.05 (1.36) \\
 & Mixtral-8x7B & 1.77 (0.19) & 14.03 (0.12) & 21.11 (1.07) & 15.50 (0.68) & 13.14 (0.83) & 18.03 (0.44) & 18.47 (0.55) \\
 & Mistral-7B &2.34 (0.17) & 22.29 (1.43) & 27.08 (0.99) & 24.15 (1.76) & 25.17 (1.74) & 26.76 (2.64) & 23.81 (2.53) \\
 & Gemma-7B & 18.87 (1.43) & 22.85 (0.81) & 22.96 (1.34) & 17.95 (0.62) & 25.46 (2.08) & 21.53 (1.00) & 17.66 (1.31) \\
 & Gemma-2B & 0.78 (0.22) & 22.99 (0.66) & 25.48 (1.54) & 25.86 (2.48) & 25.08 (1.34) & 25.21 (0.22) & 26.14 (1.71) \\
\bottomrule
\vspace{-4mm}
\end{tabular}
\end{adjustbox}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\caption{The performances of the agents on Friends dialogue in \simname (time limit = 6 seconds, with shuffled names). We conducted experiments three times and reported the accuracies and the standard deviations.}
\label{friends_shuffle_6s}
\end{table*}




==> tabs/friends_shuffle_infinite.tex <==
\begin{table*}[h]
\centering
%\small % Reduce font size
\renewcommand{\arraystretch}{1.1}
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width % \multicolumn{1}{p{2cm}}
\begin{tabular}{c l c c c c c c c} 
\toprule % \multirow{2}[7]{*}{\textbf{Model}}
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
API & GPT-4o-mini & 32.18 (1.74)$^\dagger$ & \textbf{30.27 (0.73)} & \textbf{38.40 (0.30)} & 34.70 (0.22) & 32.90 (0.57) & 36.10 (0.36) & 36.40 (0.73) \\
 \midrule
\multirow{8}{*}{Open} & \textsc{Tülu} 2-70B & 2.54 (0.21) & 26.47 (1.91) & 31.75 (1.71) & 30.94 (2.41) & 31.90 (1.25) & 29.83 (1.03) & 31.86 (2.13)\\
 & \textsc{Tülu} 2-7B & 1.15 (0.06) & 28.20 (1.63) & 27.64 (2.37) & 27.78 (1.32) & 28.98 (0.96) & 25.03 (0.94) & 29.08 (2.47)\\
 & Llama3.1-70B & 31.38 (1.01)$^\dagger$ & 29.08 (1.57) & 36.48 (2.51) & \textbf{36.91 (0.36)} & \textbf{35.89 (0.65)} & \textbf{39.80 (1.42)} & \textbf{39.00 (0.87)} \\
 & Llama3.1-8B & 27.16 (1.62)$^\dagger$ & 25.76 (1.42) & 30.61 (1.25) & 29.59 (1.25) & 30.91 (0.99) & 29.76 (1.26) & 31.59 (0.69) \\
 & Mixtral-8x7B & \textbf{34.19 (0.68)} & 25.23 (1.19) & 37.72 (0.96) & 29.48 (0.87) & 29.09 (1.46) & 31.78 (1.71) & 29.45 (0.04) \\
 & Mistral-7B & 27.78 (1.62) & 25.02 (1.26) & 30.65 (1.39) & 24.99 (1.51) & 27.34 (0.49) & 27.97 (1.31) & 26.97 (1.45) \\
 & Gemma-7B & 17.98 (2.15) & 21.64 (0.39) & 22.31 (2.15) & 18.66 (1.55) & 25.97 (1.92) & 21.79 (0.40) & 21.22 (0.59)\\
 & Gemma-2B & 1.04 (0.19) & 24.19 (0.82) & 25.25 (1.02) & 24.32 (1.55) & 25.03 (0.66) & 25.44 (1.96) & 23.62 (0.36)\\
\bottomrule
\vspace{-4mm}
\end{tabular}
\end{adjustbox}
% \vspace{-5mm}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\caption{The performances of the agents on Friends dialogue in \simname (without a time limit and with shuffled names). We conducted experiments three times and reported the accuracies and the standard deviations.}
\label{friends_shuffle_infinite}
\end{table*}

==> tabs/related_datasets.tex <==
\providecommand{\tickmark}{\ding{51}}
\providecommand{\crossmark}{\ding{55}}
\renewcommand{\arraystretch}{1.0}
\begin{table*}[t]
% \vspace{-3mm}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{l c c c c c c}
\toprule % \multirow{2}[7]{*}{\textbf{Type}} \multicolumn{1}{p{1cm}}{\centering\textbf{\# of turns$^\dagger$}}
\multirow{1}[3]{*}{\textbf{Dataset}} & \multirow{1}[3]{*}{\textbf{\# of Turns$^\dagger$}} &  \multirow{1}[3]{*}{\textbf{\# of Sessions}$^\dagger$} & \multirow{1}[3]{*}{\textbf{\# of Tokens}$^\dagger$}& \multirow{1}[3]{*}{\textbf{Collection}} & \multicolumn{1}{p{2cm}}{\centering\textbf{Avg. \#} \\ \textbf{of Speakers}} & \multicolumn{1}{p{2cm}}{\centering\textbf{Containing} \\ \textbf{QA pairs}} \\
\midrule
MSC (train; 1-4 sessions) & 53.3 & 4 & 1225.9 & Crowdsourcing & 2.0 & \crossmark \\
MSC (valid + test; 1-5 sessions) & 61.7 & 5 & 1670.9  & Crowdsourcing & 2.0 & \crossmark\\
Conversation Chronicles & 58.5 & 5 & 1054.7 & LLM & 2.0 & \crossmark \\
LoCoMo & 304.9 & 19.3 & 9209.2 & Crowdsourcing + LLM & 2.0 & \tickmark \\ \hline
\textbf{\dataname (ours)} & \textbf{18986.3} & \textbf{1313.3} & \textbf{351996.3} & \textbf{Scripts} & \textbf{3.4} & \tickmark \\
\toprule 
% \footnotesize{$\dagger$: averaged over dialogues}
\end{tabular}

\end{adjustbox}
\tiny{\makebox[\linewidth][r]{$\dagger$: averaged over dialogues}}
\vspace{-5mm}
\caption{Comparison of \dataname with other long-term dialogue datasets.}
\vspace{-5mm}
\label{tab:conversation_datasets}
\end{table*}


==> tabs/statistics.tex <==
\renewcommand{\arraystretch}{1.35}
\begin{table}[t]

%The values in parentheses for Average Question Candidates per Session refer to the number of answerable questions and unanswerable questions, respectively.
\centering
% \vspace{-1mm}
\resizebox{\linewidth}{!}{%
\begingroup
\Large % Change to desired font size (e.g., \small, \large, \scriptsize, etc.)
\begin{tabular}{lccc}
\Xhline{0.7mm}
 & \textbf{Friends} & \textbf{The Big Bang Theory} & \textbf{The Office} \\ \hline
Total \# of Tokens  & 335,439 & 367,636 & 352,914 \\ \hline
Total \# of Sessions & 788 & 805 & 2,347 \\ \hline
Fan Quiz Questions\textsuperscript{\textdagger} & 192.9 & 26.7 & 42.7 \\ \hline
TKG Questions\textsuperscript{\textdagger} & 1173.2  & 1280.1  & 455.1 \\ \hline
Question Candidates\textsuperscript{\textdagger} & 1366.1 & 1306.8  & 497.9 \\ \hline
\enspace $\hookrightarrow$Answerable Questions\textsuperscript{\textdagger} & 1215.0 & 1239.7 & 410.9 \\
\enspace $\hookrightarrow$Unanswerable Questions\textsuperscript{\textdagger} & 151.1 & 67.2 & 86.9 \\ \hline
Approx. \# of Possible Tests & $1366.1^{788}$ & $1306.8^{805}$ & $497.9^{2347}$ \\  \Xhline{0.7mm}
% \textdagger: Average number of questions per session
\end{tabular}%
\endgroup
}
\tiny{\makebox[\linewidth][r]{$\dagger$: Average number of questions per session}}
\vspace{-5mm}
\caption{Statistics of \dataname.}
\label{stattable}
\vspace{-6mm}
\end{table}


==> tabs/theoffice_original_6s.tex <==
\begin{table*}[h]
\centering
%\small % Reduce font size
\begin{adjustbox}{max width=\textwidth} % Adjust to fit within text width % \multicolumn{1}{p{2cm}}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c l c c c c c c c} 
\toprule % \multirow{2}[7]{*}{\textbf{Model}}
\multirow{4}{*}{\textbf{Type}} & \multicolumn{1}{c}{\multirow{4}{*}{\textbf{Model}}} & \multirow{4}{*}{\textbf{Base LLM}} & \multicolumn{6}{c}{\textbf{RAG-based}} \\
\cmidrule(lr){4-9}
& & & \multicolumn{3}{c}{\textbf{BM25}} & \multicolumn{3}{c}{\textbf{OpenAI Embedding}}\\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
& & & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} & \textbf{Utterance} & \textbf{Session Entire} & \textbf{Session Sum.} \\
\midrule
\multirow{3}{*}{API} & GPT-4o-mini & 28.48 (1.01)$^\dagger$ & 29.44 (0.62) & 43.16 (1.37) & 35.92 (2.50) & 37.81 (0.30) & 40.91 (0.37) & 42.83 (1.12) \\
& GPT-3.5 & \textbf{36.54 (0.32)} & \textbf{36.63 (0.57)} & 45.33 (1.00) & \textbf{40.93 (0.13)} & 42.49 (1.24) & 43.04 (0.82) & 45.18 (0.56) \\
 & Gemini 1.0 pro & 2.42 (0.18) & 35.11 (0.50) & \textbf{48.90 (1.57)} & 40.91 (0.75) & 44.72 (0.19) & 46.63 (0.89) & \textbf{45.82 (0.97)} \\
 \midrule
\multirow{9}{*}{Open} & \textsc{Tülu} 2-70B & 0.46 (0.09) & 22.33 (1.00) & 35.52 (0.89) & 23.49 (1.16) & 38.61 (1.02) & 43.49 (1.27) & 23.54 (0.52) \\
 & \textsc{Tülu} 2-7B & 0.32 (0.04) & 25.86 (0.54) & 27.95 (1.03) & 36.60 (2.11) & 22.13 (0.33) & 29.50 (0.56) & 35.51 (1.40) \\
 & Llama3.1-70B & 0.19 (0.07)$^\dagger$ & 29.21 (0.56) & 13.31 (0.94) & 21.32 (5.22) & \textbf{47.41 (0.93)} & \textbf{47.07 (1.32)} & 19.46 (1.73) \\
 & Llama3.1-8B & 21.87 (0.60)$^\dagger$ & 22.03 (0.32) & 37.94 (1.28) & 29.16 (1.80) & 27.76 (3.52) & 37.67 (1.70) & 26.67 (0.83) \\
 & Mixtral-8x7B & 1.53 (0.41) & 19.63 (0.79) & 34.35 (1.19) & 16.07 (0.56) & 20.02 (0.44) & 30.44 (1.69) & 12.43 (1.04) \\
 & Mistral-7B & 2.55 (0.09) & 30.65 (0.45) & 41.16 (1.26) & 35.67 (1.68) & 36.92 (2.13) & 42.71 (1.24) & 37.65 (2.42) \\
 & Gemma-7B & 17.81 (0.86) & 21.58 (0.61) & 25.62 (0.02) & 12.20 (0.57) & 24.88 (0.93) & 24.38 (0.52) & 15.70 (0.43) \\
 & Gemma-2B & 0.83 (0.16) & 29.71 (0.69) & 28.11 (1.14) & 34.63 (0.94) & 31.54 (0.65) & 30.31 (0.16) & 33.37 (0.27) \\
\bottomrule
\vspace{-4mm}
\end{tabular}
\end{adjustbox}
\tiny{\makebox[\linewidth][r]{$\dagger$: Both GPT-4o-mini and Llama3.1 support up to 128k tokens, but we limited them to 8k tokens due to high costs and GPU VRAM limits, respectively.}}
\caption{The performances of the agents on The Office dialogue in \simname (time limit = 6 seconds). We conducted experiments three times and reported the accuracies and the standard deviations.}
\label{theoffice_original_6s}
\end{table*}
